IsoVRBench: Video Reward Modeling Without Human Feedback

Video reward models are trained and evaluated on human preferences between videos that often differ simultaneously on properties such as prompt alignment, visual fidelity, motion, and generator identity. As a result, aggregate accuracy does not reveal which video properties a reward model can reliably distinguish. We construct preference pairs by controlled interventions that change one property of a generated video while holding the rest fixed. The resulting pairs, by construction, provide preferences for how the videos differ along a specific dimension, without requiring any human annotation. We propose IsoVRBench, a video generation reward modeling benchmark of 8,000 such pairs across eight interventions, and show that state-of-the-art models separate broad quality differences between generators but miss important features such as temporal order. The best reward model reaches only 60.8% on reordered frames against 100% for humans, and rankings on existing benchmarks do not predict this failure. Using the synthetic isolated intervation pairs as training data leads to 1) IsoVRM, a reward model outperforming its counterpart trained with a larger human labeled preference dataset by 3.8 points on VBench-2.0, 2) IsoWan, the video generator post-trained with IsoVRM, outperforming its human-data counterpart in human preferences, and 3) gains that stack when combined with human data. Because intervention pairs are automatically generated rather than collected, the benchmark and training data can be easily extended as generators evolve.

==> figs/qual_panel.tex <==

\definecolor{qramp0}{RGB}{132,190,235}
\definecolor{qramp1}{RGB}{86,158,216}
\definecolor{qramp2}{RGB}{48,124,194}
\definecolor{qramp3}{RGB}{24,94,168}
\definecolor{qramp4}{RGB}{12,64,134}
\definecolor{qramp5}{RGB}{5,36,92}
\definecolor{qred}{RGB}{178,24,43}
\definecolor{qmute}{RGB}{110,118,130}

\newlength{\qcw}\newlength{\qtot}\newlength{\qrun}\newlength{\qgap}
\setlength{\qtot}{0.925\linewidth}
\setlength{\qgap}{1pt}
\setlength{\fboxsep}{0.8pt}\setlength{\fboxrule}{1.1pt}
\setlength{\tabcolsep}{1.1pt}
\setlength{\qcw}{\dimexpr(\qtot-12\fboxsep-12\fboxrule
                  -10\tabcolsep)/6\relax}
\setlength{\qrun}{\dimexpr2\fboxsep+2\fboxrule+2\tabcolsep\relax}
\newsavebox{\qbx} \newlength{\qimh} \sbox{\qbx}{\includegraphics[width=\qcw]{figs/qual/a0.jpg}}
\setlength{\qimh}{\ht\qbx}
\newcommand{\qsep}[1]{%
  \hspace{\fboxsep}%
  {\color{#1}\rule[-\fboxsep]{\fboxrule}{\dimexpr\qimh+2\fboxsep\relax}}%
  \hspace{2\tabcolsep}%
  {\color{#1}\rule[-\fboxsep]{\fboxrule}{\dimexpr\qimh+2\fboxsep\relax}}%
  \hspace{\fboxsep}}

\newcommand{\qim}[1]{\includegraphics[width=\qcw]{figs/qual/#1.jpg}}
\newcommand{\qb}[2]{\fcolorbox{#1}{white}{\qim{#2}}}
\newcommand{\qplain}[1]{\fcolorbox{white}{white}{\qim{#1}}}
\newcommand{\qnum}[1]{{\footnotesize\color{qmute}#1}}
\newcommand{\qrow}[1]{{\small\color{qred}#1}}
\newcommand{\qhead}[3]{{\normalsize\textbf{#1}\;\qrow{#2}\quad\small #3}}
\newcommand{\qhdr}[1]{\makebox[0pt][l]{\parbox[t]{\linewidth}{#1}}}
\newcommand{\qgrp}[1]{{\small\color{qmute}\textsc{#1}}}
\newcommand{\qprompt}[1]{{\small\textit{#1}}}

\begin{tabular}{@{}cccccc@{}}
\multicolumn{6}{@{}p{\qtot}@{}}{\qgrp{prompt}\; \qprompt{Sea Monster attacking a ship full of penguins}} \\[3pt]
\multicolumn{6}{@{}l@{}}{\qhead{Anchor}{}{50 denoising steps; every row below is one change to this clip}} \\[1pt]
\qb{qramp0}{a0} & \qb{qramp1}{a1} & \qb{qramp2}{a2} & \qb{qramp3}{a3} & \qb{qramp4}{a4} & \qb{qramp5}{a5} \\
\qnum{0} & \qnum{6} & \qnum{24} & \qnum{38} & \qnum{66} & \qnum{80} \\[\qgap]
\multicolumn{6}{@{}l@{}}{\qgrp{isolated: motion}} \\[1pt]
\multicolumn{6}{@{}l@{}}{\qhdr{\qhead{\frameholdname}{held}{runs of repeated frames, each run enclosed in the color of the anchor column it freezes}}} \\[1pt]
\multicolumn{3}{@{}c}{\fcolorbox{qramp0}{white}{\qim{b0_0}\qsep{qramp0}\qim{b0_1}\qsep{qramp0}\qim{b0_2}}} & \multicolumn{1}{c}{\fcolorbox{qramp2}{white}{\qim{b0_3}}} & \multicolumn{2}{c@{}}{\fcolorbox{qramp4}{white}{\qim{b0_4}\qsep{qramp4}\qim{b0_5}}} \\
\qnum{0} & \qnum{0} & \qnum{0} & \qnum{24} & \qnum{66} & \qnum{66} \\[\qgap]
\multicolumn{6}{@{}l@{}}{\qhdr{\qhead{\temporalshufflename}{reordered}{segments reordered, all frames kept}}} \\[1pt]
\qb{qramp1}{b1_0} & \qb{qramp4}{b1_1} & \qb{qramp0}{b1_2} & \qb{qramp2}{b1_3} & \qb{qramp5}{b1_4} & \qb{qramp3}{b1_5} \\
\qnum{6} & \qnum{66} & \qnum{0} & \qnum{24} & \qnum{80} & \qnum{38} \\[\qgap]
\multicolumn{6}{@{}l@{}}{\qhdr{\qhead{\motionregenname}{regenerated}{motion between sampled frames regenerated}}} \\[1pt]
\qplain{b2_0} & \qplain{b2_1} & \qb{qred}{b2_2} & \qplain{b2_3} & \qb{qred}{b2_4} & \qplain{b2_5} \\
\qnum{key} & \qnum{key} & \qnum{\color{qred}generated} & \qnum{key} & \qnum{\color{qred}generated} & \qnum{key} \\[\qgap]
\multicolumn{6}{@{}l@{}}{\qgrp{isolated: text}} \\[1pt]
\multicolumn{6}{@{}l@{}}{\qhdr{\qhead{\attributeeditname}{edited}{one attribute rewritten, then rendered: ``\textit{\textcolor{red}{Desert Armored cyborg} attacking...}''}}} \\[1pt]
\qplain{b3_0} & \qplain{b3_1} & \qplain{b3_2} & \qplain{b3_3} & \qplain{b3_4} & \qplain{b3_5} \\
\noalign{\vskip\qgap}
\multicolumn{6}{@{}l@{}}{\qgrp{isolated: visual}} \\[1pt]
\multicolumn{6}{@{}l@{}}{\qhdr{\qhead{\reducedstepsname}{8 steps}{fewer denoising steps, prompt and seed fixed}}} \\[1pt]
\qplain{b4_0} & \qplain{b4_1} & \qplain{b4_2} & \qplain{b4_3} & \qplain{b4_4} & \qplain{b4_5} \\
\noalign{\vskip\qgap}
\multicolumn{6}{@{}l@{}}{\qgrp{not isolated: overall}} \\[1pt]
\multicolumn{6}{@{}l@{}}{\qhdr{\qhead{\alignedweakgenname}{5B, image-to-video}{5B continuing the anchor's first frame}}} \\[1pt]
\qplain{b5_0} & \qplain{b5_1} & \qplain{b5_2} & \qplain{b5_3} & \qplain{b5_4} & \qplain{b5_5} \\
\noalign{\vskip\qgap}
\multicolumn{6}{@{}l@{}}{\qhdr{\qhead{\weakgenfivename}{5B}{rendered by Wan2.2-TI2V-5B from the prompt}}} \\[1pt]
\qplain{b6_0} & \qplain{b6_1} & \qplain{b6_2} & \qplain{b6_3} & \qplain{b6_4} & \qplain{b6_5} \\
\noalign{\vskip\qgap}
\multicolumn{6}{@{}l@{}}{\qhdr{\qhead{\weakgenonename}{1.3B}{rendered by Wan2.1-T2V-1.3B}}} \\[1pt]
\qplain{b7_0} & \qplain{b7_1} & \qplain{b7_2} & \qplain{b7_3} & \qplain{b7_4} & \qplain{b7_5} \\
\noalign{\vskip\qgap}
\end{tabular}


==> figs/qual_panel_karen_revision.tex <==

\definecolor{qramp0}{RGB}{132,190,235}
\definecolor{qramp1}{RGB}{86,158,216}
\definecolor{qramp2}{RGB}{48,124,194}
\definecolor{qramp3}{RGB}{24,94,168}
\definecolor{qramp4}{RGB}{12,64,134}
\definecolor{qramp5}{RGB}{5,36,92}
\definecolor{qred}{RGB}{178,24,43}
\definecolor{qmute}{RGB}{110,118,130}

\newlength{\qcw}\newlength{\qtot}\newlength{\qrun}\newlength{\qgap}
\setlength{\qtot}{0.925\linewidth}
\setlength{\qgap}{1pt}
\setlength{\fboxsep}{0.8pt}\setlength{\fboxrule}{1.1pt}
\setlength{\tabcolsep}{1.1pt}
\setlength{\qcw}{\dimexpr(\qtot-12\fboxsep-12\fboxrule
                  -10\tabcolsep)/6\relax}
\setlength{\qrun}{\dimexpr2\fboxsep+2\fboxrule+2\tabcolsep\relax}
\newsavebox{\qbx} \newlength{\qimh} \sbox{\qbx}{\includegraphics[width=\qcw]{figs/qual/a0.jpg}}
\setlength{\qimh}{\ht\qbx}
\newcommand{\qsep}[1]{%
  \hspace{\fboxsep}%
  {\color{#1}\rule[-\fboxsep]{\fboxrule}{\dimexpr\qimh+2\fboxsep\relax}}%
  \hspace{2\tabcolsep}%
  {\color{#1}\rule[-\fboxsep]{\fboxrule}{\dimexpr\qimh+2\fboxsep\relax}}%
  \hspace{\fboxsep}}

\newcommand{\qim}[1]{\includegraphics[width=\qcw]{figs/qual/#1.jpg}}
\newcommand{\qb}[2]{\fcolorbox{#1}{white}{\qim{#2}}}
\newcommand{\qplain}[1]{\fcolorbox{white}{white}{\qim{#1}}}
\newcommand{\qnum}[1]{{\footnotesize\color{qmute}#1}}
\newcommand{\qcall}[2]{{\footnotesize\color{#1}\textbf{#2}}}
\newcommand{\qrow}[2]{{\small\color{#1}#2}}
\newcommand{\qhead}[4]{{\normalsize\textbf{#1}\;\qrow{#2}{#3}\quad\small #4}}
\newcommand{\qhdr}[1]{\makebox[0pt][l]{\parbox[t]{\linewidth}{#1}}}
\newcommand{\qgrp}[1]{{\small\color{qmute}\textsc{#1}}}
\newcommand{\qprompt}[1]{{\small\textit{#1}}}

\begin{tabular}{@{}cccccc@{}}
\multicolumn{6}{@{}p{\qtot}@{}}{\qgrp{prompt}\; \qprompt{Sea Monster attacking a ship full of penguins}} \\[3pt]
\multicolumn{6}{@{}l@{}}{\qhdr{\qhead{Anchor}{qmute}{}{50 denoising steps; frame numbers appear below}}} \\[1pt]
\qb{qramp0}{a0} & \qb{qramp1}{a1} & \qb{qramp2}{a2} & \qb{qramp3}{a3} & \qb{qramp4}{a4} & \qb{qramp5}{a5} \\
\qnum{0} & \qnum{6} & \qnum{24} & \qnum{38} & \qnum{66} & \qnum{80} \\[\qgap]
\multicolumn{6}{@{}l@{}}{\qhdr{\qhead{\framehold}{frameholdcolor}{held}{repeated frames are outlined; numbers identify the anchor frame being held}}} \\[1pt]
\qplain{b0_0} & \qb{frameholdcolor}{b0_1} & \qb{frameholdcolor}{b0_2} & \qplain{b0_3} & \qplain{b0_4} & \qb{frameholdcolor}{b0_5} \\
\qnum{0} & \qcall{frameholdcolor}{0 held} & \qcall{frameholdcolor}{0 held} & \qnum{24} & \qnum{66} & \qcall{frameholdcolor}{66 held} \\[\qgap]
\multicolumn{6}{@{}l@{}}{\qhdr{\qhead{\temporalshuffle}{temporalshufflecolor}{reordered}{all frames are reordered;}}} \\[1pt]
\qb{temporalshufflecolor}{b1_0} & \qb{temporalshufflecolor}{b1_1} & \qb{temporalshufflecolor}{b1_2} & \qb{temporalshufflecolor}{b1_3} & \qb{temporalshufflecolor}{b1_4} & \qb{temporalshufflecolor}{b1_5} \\
\qcall{temporalshufflecolor}{6} & \qcall{temporalshufflecolor}{66} & \qcall{temporalshufflecolor}{0} & \qcall{temporalshufflecolor}{24} & \qcall{temporalshufflecolor}{80} & \qcall{temporalshufflecolor}{38} \\[\qgap]
\multicolumn{6}{@{}l@{}}{\qhdr{\qhead{\motionregen}{motionregencolor}{regenerated}{outlined frames are regenerated between retained keyframes}}} \\[1pt]
\qplain{b2_0} & \qplain{b2_1} & \qb{motionregencolor}{b2_2} & \qplain{b2_3} & \qb{motionregencolor}{b2_4} & \qplain{b2_5} \\
\qnum{0 key} & \qnum{6 key} & \qcall{motionregencolor}{24 generated} & \qnum{38 key} & \qcall{motionregencolor}{66 generated} & \qnum{80 key} \\[\qgap]
\multicolumn{6}{@{}l@{}}{\qhdr{\qhead{\attributeedit}{attributeeditcolor}{edited}{all frames render the edited attribute: ``\textit{\textcolor{attributeeditcolor}{Desert Armored cyborg} attacking...}''}}} \\[1pt]
\qb{attributeeditcolor}{b3_0} & \qb{attributeeditcolor}{b3_1} & \qb{attributeeditcolor}{b3_2} & \qb{attributeeditcolor}{b3_3} & \qb{attributeeditcolor}{b3_4} & \qb{attributeeditcolor}{b3_5} \\
\qcall{attributeeditcolor}{0} & \qcall{attributeeditcolor}{6} & \qcall{attributeeditcolor}{24} & \qcall{attributeeditcolor}{38} & \qcall{attributeeditcolor}{66} & \qcall{attributeeditcolor}{80} \\[\qgap]
\multicolumn{6}{@{}l@{}}{\qhdr{\qhead{\reducedsteps}{reducedstepscolor}{8 steps}{all frames are rendered with fewer denoising steps; prompt and seed are fixed}}} \\[1pt]
\qb{reducedstepscolor}{b4_0} & \qb{reducedstepscolor}{b4_1} & \qb{reducedstepscolor}{b4_2} & \qb{reducedstepscolor}{b4_3} & \qb{reducedstepscolor}{b4_4} & \qb{reducedstepscolor}{b4_5} \\
\qcall{reducedstepscolor}{0} & \qcall{reducedstepscolor}{6} & \qcall{reducedstepscolor}{24} & \qcall{reducedstepscolor}{38} & \qcall{reducedstepscolor}{66} & \qcall{reducedstepscolor}{80} \\[\qgap]
\multicolumn{6}{@{}l@{}}{\qhdr{\qhead{\alignedweakgen}{alignedweakgencolor}{}{5B model generates continuation conditioned on the first frame. }}} \\[1pt]
\qplain{b5_0} & \qb{alignedweakgencolor}{b5_1} & \qb{alignedweakgencolor}{b5_2} & \qb{alignedweakgencolor}{b5_3} & \qb{alignedweakgencolor}{b5_4} & \qb{alignedweakgencolor}{b5_5} \\
\qnum{0 anchor} & \qcall{alignedweakgencolor}{6} & \qcall{alignedweakgencolor}{24} & \qcall{alignedweakgencolor}{38} & \qcall{alignedweakgencolor}{66} & \qcall{alignedweakgencolor}{80} \\[\qgap]
\multicolumn{6}{@{}l@{}}{\qhdr{\qhead{\weakgenfive}{weakgen5color}{}{all frames are rendered by Wan2.2-TI2V-5B from the prompt}}} \\[1pt]
\qb{weakgen5color}{b6_0} & \qb{weakgen5color}{b6_1} & \qb{weakgen5color}{b6_2} & \qb{weakgen5color}{b6_3} & \qb{weakgen5color}{b6_4} & \qb{weakgen5color}{b6_5} \\
\qcall{weakgen5color}{0} & \qcall{weakgen5color}{6} & \qcall{weakgen5color}{24} & \qcall{weakgen5color}{38} & \qcall{weakgen5color}{66} & \qcall{weakgen5color}{80} \\[\qgap]
\multicolumn{6}{@{}l@{}}{\qhdr{\qhead{\weakgenone}{weakgen13color}{}{all frames are rendered by Wan2.1-T2V-1.3B from the prompt}}} \\[1pt]
\qb{weakgen13color}{b7_0} & \qb{weakgen13color}{b7_1} & \qb{weakgen13color}{b7_2} & \qb{weakgen13color}{b7_3} & \qb{weakgen13color}{b7_4} & \qb{weakgen13color}{b7_5} \\
\qcall{weakgen13color}{0} & \qcall{weakgen13color}{6} & \qcall{weakgen13color}{24} & \qcall{weakgen13color}{38} & \qcall{weakgen13color}{66} & \qcall{weakgen13color}{80} \\[\qgap]
\end{tabular}


==> figs/teaser.tex <==
\begin{tikzpicture}[
  font=\footnotesize,
  stage/.style={draw=gray!55, rounded corners=2pt, fill=gray!4,
                minimum height=9mm, inner sep=3pt, align=center},
  video/.style={stage, minimum width=18mm},
  anchorvideo/.style={video, draw=tblhi, line width=0.8pt, fill=tblhi!7},
  variant/.style={video, draw=tbllo, line width=0.8pt, fill=tbllo!7},
  pair/.style={stage, draw=gray!65, line width=0.7pt, minimum width=25mm},
  model/.style={stage, draw=tblhi, line width=0.8pt, fill=tblhi!7,
                minimum width=23mm},
  ar/.style={-{Stealth[length=4.5pt]}, gray!70, line width=0.7pt},
]

\node[stage, text width=17mm] (prompt) at (0.75,2.25)
  {\emph{prompt}};
\node[stage, text width=18mm] (basegen) at (3.00,2.25)
  {generate};
\node[anchorvideo] (anchorvid) at (5.35,2.25)
  {anchor\\video};
\node[stage, text width=25mm] (intervention) at (7.95,2.25)
  {apply controlled\\intervention};
\node[variant] (variantvid) at (10.55,2.25)
  {modified\\video};

\draw[ar] (prompt) -- (basegen);
\draw[ar] (basegen) -- (anchorvid);
\draw[ar] (anchorvid) -- (intervention);
\draw[ar] (intervention) -- (variantvid);

\node[pair, text width=24mm] (trainpair) at (6.05,0.25)
  {\textbf{labeled video pair}\\[-1pt]
   \textcolor{tblhi}{anchor} $\succ$
   \textcolor{tbllo}{modified}};
\node[model, text width=22mm] (reward) at (8.85,0.25)
  {train video\\reward model};
\node[model, text width=24mm] (trainedgen) at (11.65,0.25)
  {reward-guided\\generator training};

\draw[ar] (anchorvid.south) -- ++(0,-0.35) -|
  ([xshift=-6mm]trainpair.north);
\draw[ar] (variantvid.south) -- ++(0,-0.35) -|
  ([xshift=6mm]trainpair.north);
\draw[ar] (trainpair) -- (reward);
\draw[ar] (reward) -- (trainedgen);

\end{tikzpicture}

